API-BLEND: A Comprehensive Corpora for Training and Benchmarking API LLMs

There is a growing need for Large Language Models (LLMs) to effectively use tools and external Application Programming Interfaces (APIs) to plan and complete tasks. As such, there is tremendous interest in methods that can acquire sufficient quantities of train and test data that involve calls to tools / APIs. Two lines of research have emerged as the predominant strategies for addressing this challenge. The first has focused on synthetic data generation techniques, while the second has involved curating task-adjacent datasets which can be transformed into API / Tool-based tasks. In this paper, we focus on the task of identifying, curating, and transforming existing datasets and, in turn, introduce API-BLEND, a large corpora for training and systematic testing of tool-augmented LLMs. The datasets mimic real-world scenarios involving API-tasks such as API / tool detection, slot filling, and sequencing of the detected APIs. We demonstrate the utility of the API-BLEND dataset for both training and benchmarking purposes.

==> sections/1-introduction.tex <==
\section{Introduction}

% The human species has achieved success primarily due to our adeptness in utilizing various tools to enhance our lives. While other living beings also exhibit this skill to some extent, humans have perfected it. Tools not only simplify our lives but also broaden our capabilities. Artificial intelligence systems must harness the full potential of the tools and APIs at their disposal instead of attempting to independently master every task.

% While Large Language Models (LLMs) have demonstrated remarkable proficiency in language understanding tasks, their ability to effectively invoke relevant APIs for accessing external tools and knowledge remains a challenge. The ability of LLMs to call external tools can significantly improve the capabilities of LLMs such as real-time information retrieval~\cite{}, knowledge graph querying~\cite{}, Reasoning~\cite{sun2023survey}. One major bottleneck for improving LLMs ability to call API is the lack of good datasets for training these models to address real-world problems. 

% One popular approach in the recent past has been synthetic data generation using larger models~\cite{wang-etal-2023-self-instruct}. These approaches start with few seed examples and use ICL prompts to generate new data with the required features.

%API-augmented LLMs will be able to precisely identify the intents in a specified sequence, accompanied by generating the correct slots and their values. Intents can be considered as function calls, where the order of execution is critical for resolving dependencies in the given problem. The slots represent the variables required by the intents. The model is also required to determine the precise values relevant to their respective slots.


The main contributions of this paper are: (1) we curate {\color{red} seven} multi-intent API datasets from existing benchmarks; (2) we showcase a novel prompt-based approach for data curation from an existing dataset using open source models; (3) we provide a comparative analysis of the features within our datasets in contrast to those in other API datasets; (4) we benchmark all the curated datasets with open-source models; and (5) we offer a detailed comparison of our fine-tuned model with other tool-based {\color{red}fine-tuned models, like ToolLLaMA}. 

We also propose a robust benchmarking approach to evaluate LLMs' performance in tool-augmented API settings. We provide a comparative analysis of state-of-the-art LLMs compared with LLMs fine-tuned using the training data. The paper provides insights into the strengths, and limitations of LLMs. We also highlight the areas for improvement in the context of the given problem. 

% * Problem statement
% * Existing approaches and the challenges (ToolAlpaca/ ToolLLM)
% * Our data-suit and quality assessments
% * Experiments and Benchmarking

%{\color{red} Please write up contributions here just a few points and I can elaborate?}
%\begin{itemize}
%    \item We introduce {\color{red}} dataset, which is the largest API-tasks dataset derived from existing benchmarks.
%    \item 
%\end{itemize}


==> sections/3-dataset-curation.tex <==
\begin{table*}[hbt!]
 \caption{Curated Datasets Statistics}
  \centering
  \scriptsize
  \begin{tabular}{lrrrrrrrr}
    \toprule
        & SeqATIS & SeqSNIPS & SeqSGD & SeqMultiWOZ & SeqTopV2 & SeqToolQA & ToolBench-HS & ToolBench-B \\
        \midrule
        TRAIN & 11670 & 39750 & 6782  & 6816 & 94458 & - & - & - \\
        DEV   & 694 & 2198 & 1092 & 485 & 13477 & - & - & - \\
        TEST  & 774 & 2199 & 1567 & 983 & 6095 & 358 & 100 & 120 \\
        \midrule
        Min. Seq-Len. & 1 & 1 & 1 & 1 & 1 & 1 & 4 & 6\\
        Max. Seq-Len. & 3 & 4 & 5 & 5 & 5 & 6 & 10 & 15 \\
        Avg. Seq-Len. & 2.13 & 1.96 & 2.44 & 2.36 & 1.2 & 2.42 & 7.01 & 9.45\\
        \midrule
        Min. No. Slots & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0\\
        Max. No. Slots & 9 & 7 & 10 & 10 & 6 & 3 & 1 & 1\\
        Avg. No. Slots & 4.85 & 5.06 & 3.5 & 3.67 & 1.98 & 1.45 & 0.86 & 0.89\\
    \bottomrule
  \end{tabular}
  \label{tab:dataset_stat}
\end{table*}



\section{Dataset Curation}

In this paper, we target a setting where the input is a single natural language utterance and the output is a sequence of API calls with their parameter names and values. We used two main approaches to create datasets, 1) using a prompt-based approach based on existing API output, and 2) heuristics-based approach to convert existing semantic parsing and personal assistant notations into API data. We detail below the steps used to create these data sets. 
Also, table~\ref{tab:dataset_stat} shows the statistics of each dataset. 








% \subsection{Prompt-based Dataset Curation}

\begin{figure*}[hbt!]
\begin{center}
\includegraphics[width=0.95\textwidth]{figures/SeqSGD.pdf}
\caption{Example of the creation process of seqSGD. Starting from the list of APIs, we use few-shot prompting to generate the summarized single utterance.}
\label{sgd_ex}
\end{center}
\end{figure*}

\subsection{SeqSGD and SeqMultiWoz}
We created SeqSGD, a dataset based on Schema-Guided Dialogue (SGD)  \cite{rastogi2020towards} dataset tailored towards API sequence evaluation. SGD contains about 20k annotated conversations between a human and a virtual assistant. These dialogues consist of engagements with various services and APIs across 20 domains, including banks, events, media, calendar, travel, and weather. To convert this dataset, for each conversation, we prompted a pretrained flan-t5-xxl\footnote{\url{https://huggingface.co/google/flan-t5-xxl}} model to convert each API into a request in natural language. We then append the corresponding text of each API to generate the summarized utterance. Figure \ref{sgd_ex} shows an example. We did not summarize the conversation itself, because it also contains API execution results, and using this as input to a summarization model resulted in many unneeded details. To make sure the generated text captures all APIs and slot values, we post-process the dataset to remove any examples where the utterance does not correctly reflect the ground truth APIs. As a result, we had approximately 6.8K train, 1.1K validation, and 1.6K test examples having an average API count of 2.44 and an average slot count per API of 3.5.     


MultiWoz~\cite{ye2021multiwoz} is another multi-domain task-oriented dialogue dataset. Following the same process of curating SeqSGD from the SGD dataset, we created SeqMultiWoz, another API dataset based on MultiWoz. The resulting dataset includes about 6.8k train, 485 validation, and 1k test samples with an average API count of 2.36 and an average slot count per API of 3.67.  

% \subsection{Programmatic Dataset Curation}
% %and SNIPS \cite{coucke2018snips} 

\subsection{SeqATIS and SeqSNIPS}

ATIS \cite{hemphill-etal-1990-atis} is a collection of human-annotated queries about flights. Queries ask for information such as flight numbers, airports, dates, times, and other relevant details. 
The dataset also provides a range of semantic labels, including intents and slot values. 
Intents are the overall goals of the queries, such as ``flight query'' or ``airfare query''. Slot values are the specific pieces of information that are being requested, such as ``departure city'' or ``arrival time''. SNIPS \cite{coucke2018snips}  is another dataset focused on voice assistants. It consists of human-annotated queries that cover various domains such as weather, music, and calendar. 

MixATIS and MixSNIPS are multi-intent datasets ~\cite{qin2020agif} built based on ATIS and SNIPS, respectively. It was created by collecting sentences from the ATIS/SNIPS dataset and connecting them with conjunctions, such as ``and''. The resulting data had sentences with 1-3 intents at a probability of 30\%, 50\%, and 20\%, respectively. 

\begin{figure*}[hbt!]
\begin{center}
\includegraphics[width=0.8\textwidth]{figures/MixSNIPS.pdf}
\caption{Example of how SeqSNIPS is created. Using a natural language utterance from MixSNIPS and the flat list of slots, we convert it into a sequence of API calls, each with a dictionary of parameter names and values.}
\label{snips_ex}
\end{center}
\end{figure*}

One issue is that they do not indicate which slots (parameters) should be associated with which intent (API). 
For example, as Figure \ref{snips_ex} shows, the original MixSNIPS dataset only evaluates model's ability to detect the two gold intents and which segments of the text are the target slots. 
To convert MixATIS and MixSNIPS datasets to a sequence of API calls, we divided utterances back to their original single intent utterances to get the corresponding slots for each intent. We then parsed its IOB (Inside/Outside/Beginning) slot notations to generate the list of API parameter names and values. Now, we merge the utterances back along with the APIs (including the parameter names and values) to get the sequence of API calls. In this way, we have curated SeqATIS and SeqSNIPS from MixATIS and MixSNIPS, respectively. In SeqATIS, we have around 11.5k train, 700 validation, and 800 test examples having an average API sequence length of 2.13 and an average slot count per API of 4.85. Whereas, SeqSNIPS consists of around 40k train, 2.2k validation, and 2.2k test samples with an average API sequence length of 1.96 and an average slot count per API of 5.06.



\subsection{SeqTopV2}
Topv2 \cite{chen-etal-2020-low-resource} is a multi-domain task-oriented semantic parsing dataset comprising examples from eight domains; alarm, event, messaging, music, navigation, reminder, timer, and weather. The total dataset consists of 180k samples, randomly divided into training, development, and test sets for each domain.
Figure~\ref{topv2_ex} shows an example from the original dataset. We followed a straightforward approach to convert this dataset into APIs using its intents ``IN:`` and slot ``SL:`` notations. Note that this dataset genuinely has a sequence of APIs that has to be followed. In the example in Figure~\ref{topv2_ex}, ``SEND\_MESSAGE`` is a subcall of ``CREATE\_REMINDER``.

The original dataset had a lot of "UNSUPPORTED" notations for examples where there is no matching intent. We excluded these cases from our API dataset. Along with them, we also removed the samples that had duplicate utterances, ambiguous intents, and analogous slot names inside the same intent. The resulting dataset is called SeqTopV2, and has 94K, 13.5K, and 6K for training, development, and testing splits, respectively. SeqTopV2 has an average API sequence length of 1.2 and an average slot count per API of 1.98.


\begin{figure*}[hbt!]
\begin{center}
\includegraphics[width=0.8\textwidth]{figures/top_v2.pdf}
\caption{Example of the creation process of SeqTopV2. Starting with the annotated semantic parse with mixed intents and slots, we convert it into a sequence of APIs. }
\label{topv2_ex}
\end{center}
\end{figure*}


\subsubsection{SeqToolQA}
ToolQA \cite{zhuang2023toolqa} is an open-source dataset designed for tool-augmented LLMs evaluation. The dataset tries to address the issue with current tool-based evaluation methods which do not distinguish between questions that can be answered using LLMs’ internal knowledge and those that require external information through tool use. 
To do so, the datasets come with 8 in-dependant datasets (e.g. Kaggle Flights, Coffee, Yelp, Airbnb, etc.) and a set of questions that can be answered only by querying those datasets, hence ruling out the internal knowledge of LLMs. The dataset is provided as a set of template-based questions with their final answers. However, it does not provide the intermediate set of steps (tools) that need to be executed to generate the answer to the given questions. The listing below shows some examples:

\begin{nolinenumbers}
\begin{lstlisting}[language=json]
{
 "qid": "easy-flight-0003", 
 "question": "What was the departure time of the 
       DL891 flight from SEA to LAX on 2022-01-22?",
 "answer": "11:54"
},
{
 "qid": "easy-dblp-0005",
 "question": "Who are the authors of An Empirical Investigation of the Optimality and Monotonicity Properties of Multiobjective Archiving Methods.?",
 "answer": "Miqing Li, Xin Yao"
}
\end{lstlisting}
\end{nolinenumbers}
In SeqToolQA, we used the provided implementation of ToolQA on how each template question is answered and transformed it into the corresponding set of tools. We show below how this is transformed {\color{red}need to elaborate}. We created a test set only from this data with a total of 358 examples from 6 domains spanning 17 different tools.

\begin{nolinenumbers}
\begin{lstlisting}[language=json,firstnumber=1]
{
 "qid": "easy-flight-0000",
 "question": "What was the departure time of the UA5480 flight from ORD to HSV on 2022-07-06?",
 "apis": [
    "LoadDB[DBName=flights]",
    "FilterDB[Origin=ORD,  Dest= HSV, FlightDate= 2022-07-06, Flight_Number_Marketing_Airline=5480, IATA_Code_Marketing_Airline=UA]",
    "GetValue[ValueName=DepTime]"
    ],
 "answer": "18:11"
},
{
 "qid": "easy-dblp-0005",
 "question": "Who are the authors of An Empirical Investigation of the Optimality and Monotonicity Properties of Multiobjective Archiving Methods.?",
 "apis": [
    "LoadGraph[GraphName=dblp]",
    "NodeCheck[GraphName=PaperNet, Node=An Empirical Investigation of the Optimality and Monotonicity Properties of Multiobjective Archiving Methods.]",
    "NodeProperty[PropertyName=authors]"
    ],
 "answer": "Miqing Li, Xin Yao"
}
\end{lstlisting}
\end{nolinenumbers}

\subsection{ToolBench}
This is a subset of ToolBench \cite{xu2023tool} focused on two domains, HomeSearch and Booking. We did not do any transformation to these datasets and rather used it ``as-is'', since they are already in API form. We show an example from this dataset.

\begin{nolinenumbers}
\begin{lstlisting}[language=json,firstnumber=1]
{
 "input": "Find a multi-family, townhouse or co-op in Cape Coral between $707000 and $1457000.",
 "apis": [
    "API.set_location("Cape Coral")",
    "API.set_buy_or_rent("buy")",
    "API.select_home_type(["Multi-family", "Townhouse", "Co-op"])",
    "API.set_min_price(707000)",
    "API.set_max_price(1457000)",
    "API.search()" 
   ]
 }
\end{lstlisting}
\end{nolinenumbers}

{\color{red}TODO: discuss further how this API is unique in the sense of how API is sequenced and why we kept it this way}

==> sections/4-data-quality.tex <==
\section{Data Quality Assessment}


\subsection{Human Evaluation}
* Fleiss Kappa scores

\subsection{LLM based evaluation}

==> sections/backup_experiments.tex <==
\section{Experiments and Results}


\begin{table*}[hbt!]
\scriptsize
\caption{Evaluation Results on \textbf{In-Distribution} datasets. Each scores are shown in the following format: \textbf{Intent-F1 | Slot-F1 | LCS-F1}. The weighted average (W. Avg.) scores are calculated using the number of test samples from table-\ref{tab:dataset_stat}.}
\centering
\begin{tabular}{c|c|ccccc|c}
FT Types                       & Models                  & {\color[HTML]{CB0000} \textbf{SeqATIS}} & {\color[HTML]{CB0000} \textbf{SeqSNIPS}} & {\color[HTML]{CB0000} \textbf{SeqSGD}} & {\color[HTML]{CB0000} \textbf{SeqMultiWOZ}} & {\color[HTML]{CB0000} \textbf{SeqTopV2}} & \textbf{W. Avg}             \\ \hline
                               & \textbf{Falcon-180B}    & 0.15 | 0.02 | 0.15                      & 0.39 | 0.07 | 0.4                        & 0.21 | 0.06 | 0.21                     & 0.44 | 0.25 | 0.45                          & 0.08 | 0 | 0.09                          & 0.19 | 0.04 | 0.2           \\
                               & \textbf{LLama-2-70B}    & 0.1 | 0.01 | 0.11                       & 0.26 | 0.03 | 0.27                       & 0.1 | 0.02 | 0.1                       & 0.23 | 0.12 | 0.25                          & 0.04 | 0 | 0.04                          & 0.11 | 0.02 | 0.12          \\
\multirow{-3}{*}{No FT}        & \textbf{ToolLLaMA-2-7B} & 0.29 | 0.03 | 0.32                      & 0.49 | 0.04 | 0.47                       & 0.43 | 0.05 | 0.45                     & 0.78 | 0.4 | 0.79                           & 0.07 | 0 | 0.08                          & 0.27 | 0.05 | 0.28          \\ \hline
                               & \textbf{Flan-t5-xxl}    & 0.92 | 0.72 | 0.92                      & 0.97 | 0.9 | 0.97                        & 0.98 | 0.69 | 0.98                     & 1 | 0.99 | 1                                & 0.96 | 0.83 | 0.96                       & 0.97 | 0.83 | 0.97          \\
                               & \textbf{StarCoder}      & 0.99 | 0.84 | 0.99                      & 0.96 | 0.87 | 0.96                       & 0.98 | 0.67 | 0.98                     & 1 | 0.99 | 1                                & 0.95 | 0.78 | 0.95                       & 0.96 | 0.8 | 0.96           \\
                               & \textbf{Facon-40b}      & 0.92 | 0.7 | 0.92                       & 0.97 | 0.89 | 0.97                       & 0.96 | 0.62 | 0.96                     & 1 | 0.97 | 1                                & 0.9 | 0.56 | 0.91                        & 0.93 | 0.67 | 0.94          \\
\multirow{-4}{*}{\shortstack{FT w. dataset \\ mentioned \\ in the column}} & \textbf{MPT-30b}        & 0.96 | 0.81 | 0.96                      & 0.97 | 0.9 | 0.97                        & 0.98 | 0.68 | 0.98                     & 1 | 0.98 | 1                                & 0.96 | 0.84 | 0.97                       & \textbf{0.97 | 0.84 | 0.97} \\ \hline
                               & \textbf{Flan-t5-xxl}    & 0.94 | 0.72 | 0.94                      & 0.96 | 0.89 | 0.97                       & 0.98 | 0.7 | 0.98                      & 1 | 0.97 | 1                                & 0.97 | 0.87 | 0.97                       & 0.97 | 0.85 | 0.97          \\
                               & \textbf{StarCoder}      & 0.98 | 0.81 | 0.98                      & 0.96 | 0.86 | 0.96                       & 0.98 | 0.67 | 0.98                     & 1 | 0.96 | 1                                & 0.96 | 0.83 | 0.96                       & 0.97 | 0.82 | 0.97          \\
                               & \textbf{Llama2-7b}      & 0.92 | 0.7 | 0.92                       & 0.96 | 0.88 | 0.97                       & 0.97 | 0.65 | 0.97                     & 1 | 0.97 | 1                                & 0.96 | 0.85 | 0.97                       & 0.96 | 0.83 | 0.97          \\
                               & \textbf{Facon-40b}      & 0.9 | 0.67 | 0.9                        & 0.96 | 0.87 | 0.97                       & 0.94 | 0.62 | 0.94                     & 1 | 0.94 | 1                                & 0.93 | 0.66 | 0.93                       & 0.94 | 0.72 | 0.94          \\
\multirow{-5}{*}{FT w. all data} & \textbf{MPT-30b}        & 0.94 | 0.77 | 0.94                      & 0.97 | 0.9 | 0.97                        & 0.98 | 0.7 | 0.98                      & 1 | 0.97 | 1                                & 0.97 | 0.87 | 0.97                       & \textbf{0.97 | 0.85 | 0.97} \\ \hline
\end{tabular}
\label{tab:in_domain_eval}
\end{table*}

\subsection{Baselines}
% \begin{itemize}
% \item LLalma2-70B \cite{touvron2023llama}
% \item Falcon 180B \cite{almazrouei2023falcon}
% \item LLAMA-2-7B \cite{touvron2023llama}
% \item FLAN-t5-XXL (11B) \cite{flan_t5}
% \item StarCoder (15B) \cite{li2023starcoder}
% \item MPT-30B \cite{mpt7b}
% \end{itemize}

In our experiments, we have used 8 open sourced models as our baselines: (1) LLaMA-2-70B \cite{touvron2023llama}, (2) Falcon-180B \cite{almazrouei2023falcon}, (3) LLAMA-2-7B \cite{touvron2023llama}, (4) Flan-T5-XXL \cite{flan_t5}, (5) Falcon-40B \cite{almazrouei2023falcon}, (6) StarCoder-15B \cite{li2023starcoder}, (7) MPT-30B \cite{mpt7b}, and (8) ToolLLaMA-2-7B \cite{qin2023toolllm}.
We train these models in three settings; (1) few shot testing: we evaluated LLAMA-2-70B, Falcon-180B, and ToolLLaMA-2-7B in a 3 shot mode; (2) Instruction fine-tuning on target dataset: we consider this setting for Flan-T5-XXL, StarCoder-15B, Falcon-40B, and MPT-30B; and (3) Instruction fine-tuning on combined datasets: we evaluated this setting for all models in (2) along with LLaMA-2-7B to evaluate whether we can get a single model trained on the plurality of all datasets and still performance well on each individual test set. For the out-of-domain experiments, we have used all the fine-tuned models from (3) in conjunction with the ToolLLaMA-2-7B, which is already fine-tuned with the ToolBench data. 

\subsection{Experimental Setup}
We have done two types of experiments with our datasets: in-domain and out-domain. In this section, we are going to discuss both of these two experiment setups along with the instructions and the training setting.

\subsubsection{Experiments on in-domain datasets}
We have done three different experiments over our five in-domain datasets, which are: SeqATIS, SeqSNIPS, SeqSGD, SeqMultiWoz, and SeqTopV2. 

\textbf{No Fine-tuning: } The first experiment we did was to check how state-of-the-art open LLMs perform in such a setting. In particular, we evaluated LLama-2-70B and Falcon-180B using 3-shot prompting. We also considered ToolLLaMA-2-7B \cite{qin2023toolllm}; a LLAMA-2-7B based model trained on API datasets generated using ChatGPT based on specifications from RapidAPIs. This model is not tuned on our own datasets, but we wanted to test the generality of such models on our own datasets. 

\textbf{Fine-tuning using one dataset}:
The next experiment we tried was to fine-tune the baselines discussed above on each dataset and test it on the corresponding test split. We have evaluated four models here: Flan-T5-XXL, StarCoder-15B, Falcon-40B, and MPT-30B. Ideally, this setting should give the best performance since the training data is focused towards one dataset and its APIs. 

\textbf{Fine-tuning on all training datasets}: In this setting, we combine all training datasets and fine-tune five models on them. The five models we have evaluated in this setting are: Flan-T5-XXL, StarCoder-15B, Falcon-40B, LLaMA-2-7B, and MPT-30B. The goal of this experiment is to check if we can get a generic model that works well when tested on each individual dataset. 

\subsubsection{Experiments on out-domain datasets}
To check the generality of the different API models, we measure the performance of all models on five out-of-domain test sets; ToolLLM, API Bank, ToolBench, our SeqToolQA and ToolAlpaca. In this experiment, we use the 5 models (i.e., Flan-T5-XXL, StarCoder-15B, Falcon-40B, MPT-30B, and LLaMA2-7B) that are fine-tuned with our combined data. In addition to these models, we have also evaluated ToolLLaMA-2-7B from ToolLLM ~\cite{qin2023toolllm} and Lynx from ToolAlpaca ~\cite{toolalpaca}. Table~\ref{tab:out_of_domain_eval} shows the results.  In this experiment, we compare the performance with 3-shot in-context learning examples for all models. 


\subsubsection{Instructions}
In all the experiments, we have used the same instructions for training and testing. We show below the instruction template. Only when evaluating non-fine-tuned models, we also provide 3 ICL examples via the part ``Here are some examples: {ICL\_EXAMPLES}'' in the instruction) and  remove it otherwise.

\begin{nolinenumbers}
\begin{lstlisting}[language=json,firstnumber=1]
### Instruction Template with ICL Examples ###
Given the APIs and Slots below, sequence them in the order in which they have to be called to answer the following query. 
Possible APIs: {INTENT_LIST} 
Possible Slots: {SLOT_LIST}
Here are some examples: {ICL_EXAMPLES}
Query: {QUERY}
Answer: 
\end{lstlisting}
\end{nolinenumbers}

\subsubsection{Settings and Parameters:}
We used QLoRA \cite{dettmers2023qlora} to fine-tune all our models. While fine-tuning the models on targeted datasets, we made sure that the model saw 100k samples in the training process. In combined data training, we fine-tuned the models for $2$ epochs over the cumulated datasets. In both cases, the batch size was $1$ with gradient accumulation steps of $8$ and a learning rate of $5e^{-5}$.

\subsection{Metrics}
To perform a fine-grained evaluation of the generated responses, we use two kinds of evaluation - sequence-wise Exact Match (EM) and normalized score. Let us assume that the gold sequence of API calls is given as $\textbf{y}=(y_0, \ldots,y_{N})$ where each $y_j=[I_j, S_j]$ representing intents and slots. The response from the model is $\hat{\textbf{y}}=(\hat{y}_0, \ldots,\hat{y}_{M})$. We use EM and normalized score to evaluate the performance of the model for three cases: intents, slots, and the overall (intents+slots). \textit{Exact match} compares if the full sequence of the response matches with the gold sequence. EM is 1 if $M=N$ and $y_k=\hat{y}_k\;\;\forall k$ and is a strict metric that checks for complete overlap of the response with the gold. \textit{Normalized score} calculates the average score of how many of the API invocations by the model match the gold responses. Therefore, normalized score $N=\sum_k \mathbbm{1}(y_k=\hat{y}_k)\;\;\forall k\in\{1..\min(N,M)\}$,  $\mathbbm{1}$ being the indicator function.

{\color{red}add LCS } We also use the Longest Common Subsequence (LCS) metric, which measures how similar two sequences are, in our case, $\textbf{y}$ and $\hat{\textbf{y}}$, the sequences of gold and predicted APIs.


\begin{table*}[hbt!]
\scriptsize
\centering
\caption{Evaluation Results on \textbf{Out-of-Distribution (OOD)} dataset. Each scores are shown in the following format: \textbf{Intent-F1 | Slot-F1 | LCS-F1}, except the ToolLLM datasets, which are intent-only, so they do not have the Slot-F1 score. All models are prompted with 3-shot examples. The weighted average (W. Avg.) scores are calculated using the number of test samples from Table ~\ref{tab:dataset_stat}.}
\begin{tabular}{c|ccccc|cc}
\toprule
                                             & \multicolumn{5}{c|}{\textbf{Fine-Tuned with all \sysname{} data}}                                                                           & \multicolumn{2}{c}{\textbf{Tool-Augmented LLMs}} \\ 
\multirow{-2}{*}{\textbf{Datasets}}          & \textbf{Facon-40b (all)} & \textbf{Flan-t5-xxl (all)}  & \textbf{MPT-30b (all)}      & \textbf{Llama2-7b (all)} & \textbf{StarCoder (all)} & \textbf{ToolLLama2-7b}    & \textbf{Lynx}        \\ \midrule
{\color[HTML]{009901} \textbf{ToolLLM-G1}}   & 0.48 | 0.47              & -                          & 0.11 | 0.11                 & 0.07 | 0.07              & 0.32 | 0.32              & 0.12 | 0.12               & 0.43 | 0.44          \\
{\color[HTML]{009901} \textbf{ToolLLM-G2}}   & 0.48 | 0.47              & -                          & 0.24 | 0.23                 & 0.09 | 0.08              & 0.53 | 0.53              & 0.01 | 0.01               & 0.33 | 0.34          \\
{\color[HTML]{009901} \textbf{ToolLLM-G3}}   & 0.5 | 0.49               & -                          & 0.51 | 0.49                 & 0.19 | 0.2               & 0.49 | 0.48              & 0.16 | 0.16               & 0.5 | 0.5            \\
{\color[HTML]{009901} \textbf{API Bank-1}}   & 0.42 | 0.15 | 0.44       & 0.57 | 0.12 | 0.59         & 0.59 | 0.21 | 0.62          & 0.52 | 0.16 | 0.55       & 0.49 | 0.15 | 0.55       & 0.11 | 0.04 | 0.12        & 0.31 | 0.11 | 0.33   \\
{\color[HTML]{009901} \textbf{API Bank-2}}   & 0.37 | 0.16 | 0.39       & 0.51 | 0.11 | 0.53         & 0.49 | 0.2 | 0.52           & 0.38 | 0.14 | 0.4        & 0.45 | 0.13 | 0.48       & 0.05 | 0.03 | 0.05        & 0.19 | 0.09 | 0.2    \\
{\color[HTML]{009901} \textbf{ToolBench-HS}} & 0.95 | 0.77 | 0.92       & 0.42 | 0.16 | 0.43         & 0.91 | 0.76 | 0.8           & 0.69 | 0.41 | 0.54       & 0.9 | 0.81 | 0.89        & 0.59 | 0.35 | 0.56        & 0.77 | 0.55 | 0.76   \\
{\color[HTML]{009901} \textbf{ToolBench-B}}  & 0.89 | 0.76 | 0.76       & 0.36 | 0.09 | 0.33         & 0.85 | 0.72 | 0.78          & 0.76 | 0.49 | 0.56       & 0.44 | 0.34 | 0.4        & 0.73 | 0.52 | 0.63        & 0.57 | 0.47 | 0.48   \\
{\color[HTML]{009901} \textbf{SeqToolQA}}    & 0.27 | 0.02 | 0.28       & 0.18 | 0 | 0.19            & 0.48 | 0.02 | 0.51          & 0.5 | 0 | 0.53           & 0.24 | 0.01 | 0.26       & 0.14 | 0 | 0.14           & 0.27 | 0.02 | 0.29   \\
{\color[HTML]{009901} \textbf{ToolAlpaca}}   & 0.38 | 0.07 | 0.38       & 0.56 | 0.14 | 0.57         & 0.45 | 0.11 | 0.45          & 0.55 | 0.12 | 0.56       & 0.52 | 0.16 | 0.53       & 0.01 | 0 | 0.01           & 0.01 | 0 | 0.01      \\ \hdashline
\textbf{W. Avg.}                             & 0.46 | 0.21 | 0.46       & 0.42 | 0.09 | 0.43         & \textbf{0.48 | 0.23 | 0.48} & 0.42 | 0.16 | 0.41       & 0.45 | 0.18 | 0.46       & 0.16 | 0.09 | 0.16        & 0.33 | 0.13 | 0.33  \\
\bottomrule
\end{tabular}
\label{tab:out_of_domain_eval}
\end{table*}


%=========================================





\subsection{Results on in-domain datasets}
The in-domain results on five datasets: SeqATIS, SeqSNIPS, SeqSGD, SeqMultiWoz, and SeqTopV2 are demonstrated in table \ref{tab:in_domain_eval}. 

\textbf{No Fine-tuning evaluation}: 
% The first experiment we did was to check how state-of-the-art open LLMs perform in such a setting. In particular, we evaluated LLama-2-70B and Falcon-180B using 3-shot prompting. We also considered ToolLLaMA-2-7B \cite{qin2023toolllm}; a LLAMA-2-7B based model trained on API datasets generated using ChatGPT based on specifications from RapidAPIs. This model is not tuned on our own datasets, but we wanted to test the generality of such model on our own datasets. 
On all datasets, all three non-fine-tunned models seem to get some of the intents/APIs correctly but fail to get the slots to call such APIs and hence the overall scores which check for both intents and slots are almost zero in all the cases. 

\textbf{Fine-tuning using one dataset}:
% The next experiment we tried was to fine-tune the baselines discussed above on each dataset and test it on the corresponding test split. Ideally, this should give the best performance since the training data is focused towards one dataset and its APIs. 
In this experiment, all models achieved very good performance ($>$ 90\%) detecting the right intents with the performance of all models reaching 100\% exact match on intents for SeqMultiWoz datasets. We think the reason for such performance is the fact that the number of intents in most datasets is not very large (12 intents for SeqMultiWoz). Detecting the correct set of slot names and values is a more challenging problem for most models with performance being the lowest for the SeqSGD dataset. Overall numbers suggest that Flan-T5-XXL and MPT-30B achieve the first and second-best numbers on the majority of the datasets. 


\textbf{Fine-tuning on all training datasets}: 
%In this setting, we combine all training datasets and fine-tune each model on it. The goal of this experiment is to check if we can get a generic model that works well when tested on each individual dataset. 
As shown in Table \ref{tab:in_domain_eval}, on SeqATIS and SeqMultiWoz, models trained on the combined training data achieve lower performance compared to models trained on the specific dataset. Performance on SeqSNIPS was similar for both models, while models trained on the combined data achieved better performance on SeqSGD and SeqTopV2.  

\subsection{Results on out-of-domain datasets}
% We measure the performance of all models on three out-of-domain test sets; SeqToolQA and two subsets from ToolBench; HomeSearch and Booking. In this experiment, we use the 5 models (i.e., Flan-T5-XXL, StarCoder-15B, Falcon-40B, MPT-30B, and LLaMA2-7B) that are fine-tuned with our combined data (presented in Table \ref{tab:results}). In addition to these models, we have also evaluated ToolLLaMA-2-7B on our out-of-domain test sets.  In this experiment, we compare the performance with 3-shot in-context learning examples for all models. 
Table \ref{tab:out_of_domain_eval} showcases the evaluation results for three out-of-domain datasets (i.e., SeqToolQA, ToolBench-HomeSearch, and ToolBench-Booking). Models fine-tuned on our data achieve generally better performance over ToolLLaMA-2-7B. The results seem to favor us due to the fact that the instructions used for training our models are the same as the instructions used for testing; whereas, the ToolLLaMA was fine-tuned with different instructions. On SeqToolQA, even if the models have scored some points in intent detection, however, all the models performed very poorly on detecting the slot names and values, which leads to zero overall scores. This is because the slot values in SeqToolQA contain Python codes, SQL queries, math functions, etc., which models have not seen in any training data, and these special slot values are not trivial to generate by seeing only a few ICL examples. On ToolBench test sets, the LLaMA-2-7B performs poorly in both cases, whereas StarCoder-15B and MPT-30B are doing the best on HomeSearch and Booking test sets, respectively. 

\subsection{Qualitative Studies}
We have done extensive studies on the outputs generated by the models in our experiments. In this section, we are going to discuss our findings on the failed cases along with some common mistakes demonstrated by the models. We found, in most of the cases, the issues are with the slot names and values and that is the obvious reason for not doing well on slots in both in and out-domain test sets. We provide samples for each case for better understanding. We would like to mention that most of the provided examples contain ``gold\_output'' and ``predicted\_output'' and we have shown only the error part (sub-string) from the original outputs.



\subsubsection{Parsing Issues}
Parsing challenges are the most commonly found issues in all the test cases. We have not done any post-processing on the generated text and compared the generated text directly with the gold output. This is because, we want to build a generic model that can work on any out-of-domain blind test sets, if we start fixing on a case-by-case basis, the models will be biased towards our in and out-domain datasets. 

\textbf{Space Mismatch}: This happens when the gold output and generated texts have exact same words with different numbers of spaces in between and that creates an error when we calculate an exact match scores. In the following example, we can see a space mismatch between `=' and ` = '.

\begin{nolinenumbers}
\begin{lstlisting}[language=json,firstnumber=1]
### SeqToolQA ###
{
 "gold": "NodeProperty(PropertyName=keywords)",
 "predicted":"NodeProperty(PropertyName = keywords)"
}
\end{lstlisting}
\end{nolinenumbers}

\textbf{Quotation Mismatch}: The mismatch occurs when the gold\_output and the predicted texts use different types of quotation marks. In the below example, the gold\_output uses double quotes whereas the generated text uses a single quote.

\begin{nolinenumbers}
\begin{lstlisting}[language=json,firstnumber=1]
### ToolBench ###
{
 "gold": "select_booking_type(\"trip tickets\")",
 "predicted": "select_booking_type('trip tickets')"
}
\end{lstlisting}
\end{nolinenumbers}

\subsubsection{Unnormalized Slot-Values}
In an ideal scenario, the slot values should be extracted exactly from the query by the models while generating the texts. However, sometimes, the model extracts the sub-part of it or represents it in a different form after extracting it. In a human evaluation, we would consider the generated text matches the gold, although while doing it programmatically it's showing a mismatch and we have not found a good way to normalize the slot values. The following examples capture some of the unnormalized slot value mismatches. In the first and second examples, we can see the month and the day in the predicted output are repeating. The predicted output on the third one contains only the city name, whereas the gold contains the city and the state. In the final example, even if the intent and slot values are correct, they have used different argument formats to represent it.   

\begin{nolinenumbers}
\begin{lstlisting}[language=json,firstnumber=1]
### SeqSGD ###
{                   
   "gold": "March 3rd, this Sunday",
   "predicted": "March 3rd, the 3rd"
}
{
   "gold": "March 4th",
   "predicted": "4th of March, March 4th"
}
{
   "gold": "NYC, New York",
   "predicted": "NYC"
}

### ToolBench ###
{
   "gold": "Date(3, 9, 2023)",
   "predicted": "Date(year=2023, month=3, day=9)"
}
\end{lstlisting}
\end{nolinenumbers}

\subsubsection{Semantically similar slot-names in API Specification}
In our instructions, we are providing the possible list of intents and slots to be used by the model while answering the queries. We extract these intents and slots from the original dataset's API specifications. However, we found in some cases the slot names are semantically very similar. Here is an API specification example of the `FindBus' intent along with the parameters (i.e. slots).

\begin{nolinenumbers}
\begin{lstlisting}[language=json,firstnumber=1]
### SeqSGD ###
"FindBus": {
    "description": "Search for a bus itinerary between two places on a certain date",
    "parameters": [
            "from_location",
            "leaving_date",
            "leaving_time",
            "to_location",
            "travelers",
            "departure_date",
            "departure_time",
            "from_city",
            "num_passengers",
            "to_city",
            "category",
            "destination",
            "fare_type",
            "origin",
            "group_size"
    ]
}
\end{lstlisting}
\end{nolinenumbers}

As we can see in the above list of parameters (slots) that many parameters are very similar. Here are the 4 such cases: (1) \textit{leaving\_date} and \textit{departure\_date}; (2) \textit{leaving\_time} and \textit{departure\_time}; (3) \textit{origin}, \textit{from\_city}, and \textit{from\_location}; and (4)
\textit{destination}, \textit{to\_city}, and \textit{to\_location}. Now, it often happens that the slot values are correct in the generated text but the slot names do not exactly match with the gold, even if they are very close. Following are some examples of such cases.


\begin{nolinenumbers}
\begin{lstlisting}[language=json,firstnumber=1]
### SeqSGD ###
{
  "gold": "destination_airport = ATL",
  "predicted": "destination = ATL"
}
{
  "gold": "origin_airport = LA",
  "predicted": "origin = LA"
}
{
  "gold": "show_type = imax",
  "predicted": "theater_name = imax"
}

### SeqATIS ###
{
   "gold": "cuisine = souvlaki",
   "predicted": "served_dish = souvlaki"
}
\end{lstlisting}
\end{nolinenumbers}

% \subsection{How good these models generalize?}
% * transfer learning experiments

% \subsection{Ablation Study}
% * Remove slots from the datasets, how good the models are with only intents?
 





% \begin{table}[t!]
% \scriptsize
% \caption{Evaluation Results on Out-of-Distribution (OOD) dataset. Here, \textbf{N. Sc.} means \textbf{Normalized Score}, \textbf{EM} means \textbf{\textit{Exact Match}}, and \textbf{FT} means \textbf{\textit{Fine-Tuning}}. All models are prompted with 3-shot examples.}
% \centering
% \begin{tabular}{llrrrrrrr}
%     & \multirow{2}{*}{Models} & \multicolumn{2}{c}{Intent} & \multicolumn{2}{c}{Slots} & \multicolumn{2}{c}{Overall} &  \multirow{2}{*}{LCS F1} \\
%     & & N. Sc. & EM & N. Sc. & EM & N. Sc. & EM &\\ 
% \midrule
% \midrule
% \multirow{8}{*}{SeqToolQA}  & Falcon-180B   & & & & & & &\\
%                          & LLalma-70B & & & & & & &\\
%                          & ToolLLaMA  & 0.1 & 0 & 0 & 0 & 0 & 0 &  0.002\\
%                          & Flan-T5-XXL (FT w. SeqAPI data)  & 0.35 & 0.31 & 0 & 0 & 0 & 0 & 0.003\\
%                          & StarCoder-15B (FT w. SeqAPI data) & 0.21 & 0.05 & 0.02 & 0 & 0.01 & 0 & 0.006\\
%                          & Falcon-40B (FT w. SeqAPI data) & 0.34 & 0.14 & 0.04 & 0 & 0.02 & 0 & 0.014\\
%                          & MPT-30B (FT w. SeqAPI data) & 0.59 & 0.53 & 0.02 & 0 & 0.01 & 0 &  0.010\\
%                          & LLaMA2-7B (FT w. SeqAPI data) & 0.66 & 0.65 & 0.01 & 0.01 & 0 & 0 & 0.000\\
% \midrule
% \multirow{8}{*}{ToolBench-HomeSearch}  & Falcon-180B (3 shots)  & & & & & & &\\
%                          & LLalma-70B  & & & & & & &\\
%                          & ToolLLaMA  & 0.6 & 0.18 & 0.36 & 0 & 0.36 & 0 & \\
%                          & Flan-T5-XXL (FT w. SeqAPI data) & 0.98 & 0.92 & 0.22 & 0.04 & 0.24 & 0.04 & \\
%                          & StarCoder-15B (FT w. SeqAPI data) & 0.91 & 0.68 & 0.83 & 0.48 & 0.83 & 0.48 & \\
%                          & Falcon-40B (FT w. SeqAPI data) & 0.97 & 0.78 & 0.83 & 0.21 & 0.83 & 0.21 & \\
%                          & MPT-30B (FT w. SeqAPI data) & 0.96 & 0.78 & 0.86 & 0.33 & 0.87 & 0.33 & \\
%                          & LLaMA2-7B (FT w. SeqAPI data) & 0.73 & 0.21 & 0.54 & 0.03 & 0.54 & 0.03 & \\
% \midrule
% \multirow{8}{*}{ToolBench-Booking}  & Falcon-180B   & & & & & & &\\
%                          & LLalma-70B  & & & & & & &\\
%                          & ToolLLaMA  & 0.69 & 0.01 & 0.6 & 0.01 & 0.47 & 0 &  \\
%                          & Flan-T5-XXL (FT w. SeqAPI data) & 0.94 & 0.75 & 0.28 & 0.15 & 0.29 & 0.15 & \\
%                          & StarCoder-15B (FT w. SeqAPI data) & 0.45 & 0.22 & 0.41 & 0.11 & 0.39 & 0.08 & \\
%                          & Falcon-40B (FT w. SeqAPI data) & 0.92 & 0.55 & 0.9 & 0.37 & 0.81 & 0.22 & \\
%                          & MPT-30B (FT w. SeqAPI data) & 0.92 & 0.53 & 0.85 & 0.37 & 0.83 & 0.32 & \\
%                          & LLaMA2-7B (FT w. SeqAPI data) & 0.82 & 0.33 & 0.61 & 0.08 & 0.42 & 0 & \\
% \midrule
% \bottomrule
% \end{tabular}

% \label{tab:results_ood}
% \end{table}

% \begin{table}[t!]
% \scriptsize
% \caption{Evaluation Results on Curated Datasets. Here, \textbf{N. Sc.} means \textbf{Normalized Score}, \textbf{EM} means \textbf{\textit{Exact Match}}, and \textbf{FT} means \textbf{\textit{Fine-Tuning}}.}
% \centering
% % \begin{tabular}{l|l|l|rr|rr|rr|rr}
% \begin{tabular}{lllrrrrrrrr}
%     & \multirow{2}{*}{FT Types} & \multirow{2}{*}{Models} & \multicolumn{2}{c}{Intent} & \multicolumn{2}{c}{Slots} & \multicolumn{2}{c}{Overall} & \multirow{2}{*}{Set F1} & \multirow{2}{*}{LCS F1} \\
%     & & & N. Sc. & EM & N. Sc. & EM & N. Sc. & EM & &\\ 
% \midrule
% \midrule
% \multirow{11}{*}{SeqATIS} & \multirow{2}{*}{NO-FT} & Falcon-180B  & 0.17 & 0.11 & 0.02 & 0 & 0.02 & 0 & 0.01 & 0.01\\
%                          & & LLalma-70B & 0.13 & 0.1 & 0.02 & 0 & 0.01 & 0 & 0.006& 0.006\\
%                          & & ToolLLaMA & 0.29 & 0.13 & 0.04 & 0.01 & 0.03 & 0.01 &  &  \\\cmidrule{2-11}
%                          & \multirow{4}{*}{FT w. SeqATIS} & Flan-T5-XXL   & 0.93 & 0.84 & 0.77 & 0.5 & 0.71 & 0.5 & 0.71 & 0.71\\
%                          & & StarCoder-15B   & 1 & 0.99 & 0.85 & 0.62 & 0.78 & \textbf{0.62} & 0.78 & 0.78 \\
%                          & & Falcon-40B  & 0.92 & 0.84 & 0.75 & 0.43 & 0.64 & 0.41 & 0.64 & 0.64 \\
%                          & & MPT-30B  & 0.96 & 0.92 & 0.85 & 0.62 & 0.79 & 0.61 & \textbf{0.79} & \textbf{0.79} \\ \cmidrule{2-11}
%                          & \multirow{5}{*}{FT w. all data} & Flan-T5-XXL & 0.94 & 0.88 & 0.75 & 0.45 & 0.68 & 0.45 & 0.68 & 0.68\\
%                          & & StarCoder-15B & 0.98 & 0.97 & 0.82 & 0.56 & 0.74 & 0.54 & 0.74 & 0.74 \\
%                          & & LLaMA2-7B & 0.92 & 0.84 & 0.76 & 0.45 & 0.66 & 0.44 & 0.66 & 0.66 \\
%                          & & Falcon-40B & 0.9 & 0.81 & 0.73 & 0.43 & 0.64 & 0.42 &  &  \\
%                          & & MPT-30B & 0.94 & 0.88 & 0.82 & 0.53 & 0.73 & 0.53 &  &  \\
% \midrule
% \multirow{11}{*}{SeqSNIPS} & \multirow{2}{*}{NO-FT} & Falcon-180B  & 0.42 & 0.30 & 0.01 & 0.00 & 0.01 &0.00  & 0.007 &0.007\\
%                          & & LLalma-70B & 0.30 & 0.20 &0.01  & 0.00& 0.00 & 0.00 & 0.005 &  0.005\\ 
%                          & & ToolLLaMA & 0.41 & 0.14 & 0.01 & 0 & 0 & 0 &  &   \\\cmidrule{2-11}
%                          & \multirow{4}{*}{FT w. SeqSNIPS} & Flan-T5-XXL   & 0.96 & 0.92 & 0.92 & 0.77 & 0.86 & \textbf{0.75} & \textbf{0.87} & \textbf{0.87} \\
%                          & &StarCoder-15B  & 0.95 & 0.91 & 0.91 & 0.7 & 0.82 & 0.69 & 0.83 & 0.83 \\
%                          & & Falcon-40B  & 0.96 & 0.92 & 0.93 & 0.77 & 0.86 & \textbf{0.75} & \textbf{0.87} & \textbf{0.87}\\
%                          & & MPT-30B  & 0.96 & 0.92 & 0.93 & 0.77 & 0.87 & \textbf{0.75} & \textbf{0.87} & \textbf{0.87} \\ \cmidrule{2-11}
%                          & \multirow{5}{*}{FT w. all data} & Flan-T5-XXL & 0.96 & 0.91 & 0.92 & 0.74 & 0.85 & 0.73 & 0.86 & 0.86\\
%                          & & StarCoder-15B & 0.95 & 0.91 & 0.9 & 0.68 & 0.81 & 0.66 & 0.82 & 0.82 \\
%                          & & LLaMA2-7B & 0.96 & 0.92 & 0.92 & 0.74 & 0.84 & 0.71 & 0.85 & 0.85 \\
%                          & & Falcon-40B & 0.96 & 0.91 & 0.91 & 0.73 & 0.81 & 0.67 &  &  \\
%                          & & MPT-30B & 0.96 & 0.92 & 0.92 & 0.76 & 0.86 & 0.75 &  &  \\
% \midrule
% \multirow{11}{*}{SeqSGD} & \multirow{2}{*}{NO-FT} & Falcon-180B  & 0.22 & 0.16 & 0.02 & 0 & 0.02 & 0 &0.013 & 0.013\\
%                          & & LLalma-70B & 0.11 & 0.08 & 0.01 & 0 & 0.01 & 0 & 0.001&0.001\\ 
%                          & & ToolLLaMA & 0.37 & 0.1 & 0.02 & 0 & 0.02 & 0 &  &  \\\cmidrule{2-11}
%                          & \multirow{4}{*}{FT w. SeqSGD} & Flan-T5-XXL   & 0.98 & 0.96 & 0.62 & 0.23 & 0.42 & 0.22 & 0.42 & 0.42 \\
%                          & & StarCoder-15B  & 0.98 & 0.96 & 0.6 & 0.22 & 0.39 & 0.2 & 0.39 & 0.39 \\
%                          & & Falcon-40B  & 0.97 & 0.94 & 0.59 & 0.22 & 0.33 & 0.15 & 0.33 & 0.33 \\
%                          & & MPT-30B  & 0.98 & 0.96 & 0.63 & 0.26 & 0.42 & 0.23 & 0.42 & 0.42 \\ \cmidrule{2-11}
%                          & \multirow{5}{*}{FT w. all data} & Flan-T5-XXL & 0.98 & 0.95 & 0.64 & 0.29 & 0.43 & \textbf{0.24} & \textbf{0.43} & \textbf{0.43}\\
%                          & & StarCoder-15B & 0.98 & 0.97 & 0.61 & 0.21 & 0.37 & 0.18 & 0.37 & 0.37 \\
%                          & & LLaMA2-7B & 0.97 & 0.93 & 0.61 & 0.22 & 0.36 & 0.18 & 0.36 & 0.36 \\
%                          & & Falcon-40B & 0.94 & 0.88 & 0.61 & 0.19 & 0.31 & 0.13 &  & \\
%                          & & MPT-30B & 0.99 & 0.97 & 0.64 & 0.25 & 0.4 & 0.2 &  &  \\
% \midrule
% \multirow{11}{*}{SeqMultiWOZ} & \multirow{2}{*}{NO-FT} & Falcon-180B  & 0.47 & 0.4 & 0.3 & 0.07 & 0.01 & 0 &0.01 &0.01\\
%                          & & LLalma-70B & 0.32 & 0.29 & 0.19 & 0.09 & 0.01 & 0.01 & 0.008&0.008\\ 
%                          & & ToolLLaMA & 0.72 & 0.36 & 0.42 & 0.02 & 0.01 & 0 &  &  \\\cmidrule{2-11}
%                          & \multirow{4}{*}{FT w. SeqMultiWOZ} & Flan-T5-XXL   & 1 & 1 & 0.99 & 0.92 & 0.93 & \textbf{0.86} & \textbf{0.93} & \textbf{0.93} \\
%                          & & StarCoder-15B  & 1 & 1 & 0.99 & 0.89 & 0.93 & \textbf{0.86} & \textbf{0.93} & \textbf{0.93} \\
%                          & & Falcon-40B  & 1 & 1 & 0.98 & 0.83 & 0.86 & 0.74 & 0.86 & 0.86 \\
%                          & & MPT-30B  & 1 & 1 & 0.98 & 0.88 & 0.91 & 0.83 & 0.91 & 0.91 \\ \cmidrule{2-11}
%                          & \multirow{5}{*}{FT w. all data} & Flan-T5-XXL & 1 & 1 & 0.97 & 0.79 & 0.87 & 0.74 & 0.87 & 0.87\\
%                          & & StarCoder-15B & 1 & 1 & 0.97 & 0.78 & 0.84 & 0.69 & 0.84 & 0.84 \\
%                          & & LLaMA2-7B & 1 & 1 & 0.97 & 0.78 & 0.85 & 0.71 & 0.85 & 0.85 \\
%                          & & Falcon-40B & 1 & 0.99 & 0.95 & 0.68 & 0.77 & 0.56 &  & \\
%                          & & MPT-30B & 1 & 1 & 0.98 & 0.83 & 0.88 & 0.76 &  &  \\
% \midrule
% \multirow{11}{*}{SeqTopV2} & \multirow{2}{*}{NO-FT} & Falcon-180B  & 0.04 & 0.03 &0.00 & 0.00& 0.00& 0.00& 0.001&0.001\\
%                          & & LLalma-70B & 0.08 & 0.06 &0.00 & 0.00& 0.00& 0.00& 0.001&0.001\\
%                          & & ToolLLaMA & 0.05 & 0 & 0 & 0 & 0 & 0 &  &  \\\cmidrule{2-11}
%                          & \multirow{4}{*}{FT w. SeqTopV2} & Flan-T5-XXL   &0.97 & 0.96 & 0.87 & 0.8 & 0.8 & 0.78 & 0.8 & 0.8 \\
%                          & & StarCoder-15B  & 0.96 & 0.95 & 0.84 & 0.76 & 0.75 & 0.73 & 0.75 & 0.75 \\
%                          & & Falcon-40B  & 0.94 & 0.93 & 0.68 & 0.6 & 0.53 & 0.52 & 0.53 & 0.53 \\
%                          & & MPT-30B  & 0.97 & 0.97 & 0.89 & 0.83 & 0.81 & 0.8 & 0.81 & 0.81 \\ \cmidrule{2-11}
%                          & \multirow{5}{*}{FT w. all data} & Flan-T5-XXL & 0.97 & 0.97 & 0.9 & 0.84 & 0.84 & 0.82 & \textbf{0.84} & \textbf{ 0.84} \\
%                          & & StarCoder-15B & 0.97 & 0.96 & 0.88 & 0.82 & 0.81 & 0.79 & 0.81 & 0.81 \\
%                          & & LLaMA2-7B & 0.97 & 0.97 & 0.9 & 0.85 & 0.84 & \textbf{0.83} & \textbf{0.84} & \textbf{0.84} \\
%                          & & Falcon-40B & 0.94 & 0.93 & 0.68 & 0.6 & 0.53 & 0.52 &  &  \\
%                          & & MPT-30B & 0.97 & 0.97 & 0.89 & 0.83 & 0.81 & 0.8 &  &  \\

% \midrule
% \bottomrule
% \end{tabular}

% \label{tab:results}
% \end{table}



